Tensor Convolutional Network for Higher-Order Interaction Prediction in Sparse Tensors

Many real-world data, such as recommendation data and temporal graphs, can be represented as incomplete sparse tensors where most entries are unobserved. For such sparse tensors, identifying the top-k higher-order interactions that are most likely to occur among unobserved ones is crucial. Tensor factorization (TF) has gained significant attention in various tensor-based applications, serving as an effective method for finding these top-k potential interactions. However, existing TF methods primarily focus on effectively fusing latent vectors of entities, which limits their expressiveness. Since most entities in sparse tensors have only a few interactions, their latent representations are often insufficiently trained. In this paper, we propose TCN, an accurate and compatible tensor convolutional network that integrates seamlessly with existing TF methods for predicting higher-order interactions. We design a highly effective encoder to generate expressive latent vectors of entities. To achieve this, we propose to (1) construct a graph structure derived from a sparse tensor and (2) develop a relation-aware encoder, TCN, that learns latent representations of entities by leveraging the graph structure. Since TCN complements traditional TF methods, we seamlessly integrate TCN with existing TF methods, enhancing the performance of predicting top-k interactions. Extensive experiments show that TCN integrated with a TF method outperforms competitors, including TF methods and a hyperedge prediction method. Moreover, TCN is broadly compatible with various TF methods and GNNs (Graph Neural Networks), making it a versatile solution.

==> 070application.tex <==


\begin{table*}[t!]
%	\vspace{-2mm}
	\caption{Description of real-world tensor datasets.
%	in $\mathbb{R}^{t \times c}$ where $t$ corresponds to total length (time), and $c$ corresponds to the number of time series.
	}
	\centering
	\label{tab:Description}
		\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lrrrrrrrc}
		\toprule
		& \multicolumn{3}{c}{\textbf{Total Tensor Size}} & \multicolumn{3}{c}{\textbf{Initial Tensor Size}} & \\
		\textbf{Dataset} & \textbf{Max Dim. $I_k$} & \textbf{Dim. $J$} & \textbf{Dim. $K$} & \textbf{Max Dim. $I_k$} & \textbf{Dim. $J$} & \textbf{Dim. $K$} & \textbf{Update Cycle} & \textbf{Newly Arrived Data} \\
		\midrule
%		 Brainq\footnoteref{foot:brainq}~\cite{MitchellT2008Predicting}  & $3$ & $(360, 21764, 9)$ & $(10, 10, 5)$ \\
		US Stock~\cite{JangK22} &  $7,397$ & $85$ & $4,742$ &  $1,458$ & $85$ & $994$ & 60 days & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}New rows of existing slice matrices \\ and new slice matrices \blue{arrive}\end{tabular}} \\
		KR Stock~\cite{JangK21} &  $5,268$ & $85$ & $3,620$ &  $995$ & $85$ & $2,092$ & 60 days  \\
		\midrule
		JPN Stock &  $2,204$ & $85$ & $215$ &  $424$ & $85$ & $215$  & 20 days & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}New rows of \\ existing slice matrices \blue{arrive}\end{tabular}} \\
		CHN Stock &  $2,431$ & $85$ & $219$ &  $471$ & $85$ & $219$  & 20 days \\						
		VicRoads~\cite{schimbinschi2015traffic} &  $1,084$ & $96$ & $2,033$ &  $184$ & $96$ & $2,033$  & 20 days \\					
		PEMS &  $440$ & $144$ & $963$ &  $80$ & $144$ & $963$  & 20 days \\						
		\bottomrule
	\end{tabular}}
\end{table*}



What anomalies exist in a dual-way streaming setting?
How can we find them using \method?
As new rows of slice matrices and new slice matrices \blue{arrive} over time, various anomalies are hidden in the new ones.
Although factor matrices are updated using the new incoming data, anomalies are still very different from predictions by the updated factor matrices.
\method efficiently finds anomalies by measuring reconstruction errors with updated factor matrices.

\blue{We find two types of anomaly detection in our dual-way streaming setting:}
\begin{enumerate}
%	\item \textbf{Element-level anomaly detection.} We measure element-wise reconstruction errors and then find an update cycle that provokes \blue{a large error} from the previous update.
	\item \textbf{Slice-level anomaly detection.}	 For a slice matrix, we measure slice matrix-wise reconstruction errors and then find \blue{an update that provokes a large error.}
	\item \textbf{Tensor-level anomaly detection.}	 We measure the reconstruction error for a newly arrived tensor and then compare it \blue{with a threshold.}
\end{enumerate}


%
%\textbf{Element-level anomaly detection.}
%We find element-level anomalies by measuring reconstruction errors of elements of a new incoming tensor and comparing them.
%\blue{For an element, we regard the updates that have high reconstruction errors as anomalies.}
%The following definition is an element-level reconstruction error used for detecting element-level anomalies:
%\begin{definition}[Element-level reconstruction error]
%		When a new element $\mat{X}_{k,new}(i,j)$ is given, an element-level reconstruction error is as follows:
%\blue{\begin{align}
%	ee\left(\mat{X}_{k,new}(i,j)\right) = |\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|
%\end{align}
%where $|\mat{X}(i,j)-\hat{\mat{X}}(i,j)|$ indicates the absolute value of $\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)$.}
%\end{definition}

\textbf{Slice-level anomaly detection.}
\blue{
We find slice-level anomalies by measuring reconstruction errors of slice matrices and investigating them independently.}
We compute reconstruction errors of slice matrices based on the following definition:
\begin{definition}[Slice-level reconstruction error]
\label{def:slice_level}
		When a newly arrived slice matrix $\mat{X}_{k,new}$ is given, a slice-level reconstruction error is as follows:
\blue{
\begin{align}
	se\left(\mat{X}_{k,new}\right) = \frac{1}{I_{k,new}\times J}{\sum_{i,j}{{|\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|}}}
\end{align}
where $\hat{\mat{X}}_{k,new}$ is the reconstructed matrix by $\mat{U}_{k,new}\mat{S}_{k,new}\mat{V}_{new}^T$.
}
\end{definition}




\textbf{Tensor-level anomaly detection.}
We detect tensor-level anomalies by measuring a reconstruction error for a newly arrived tensor.
There are newly arrived tensors that fail to be reconstructed well.
\blue{When a new tensor arrives}, we obtain a reconstruction error by updating factor matrices and comparing the new one with the reconstructed data by the updated factor matrices.
Then, we compare it with reconstruction errors measured at previous updates.
The following definition presents the tensor-level reconstruction error:
\begin{definition}[Tensor-level reconstruction error]
\label{def:tensor_level}
		When a newly arrived tensor $\T{X}_{new} = \{\mat{X}_{k,new}\}_{k=1}^{K+L}$ is given, tensor-level reconstruction error is as follows:
\blue{
\begin{align}
\begin{split}
	& te\left(\{\mat{X}_{k,new}\}_{k=1}^{K+L}\right) = \\
	&  \frac{1}{K+L}\sum_{k=1}^{K+L}\frac{1}{I_{k,new}\times J}{\sum_{i,j}{|\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|}}
\end{split}
\end{align}
where $\hat{\mat{X}}_{k,new}$ is reconstructed by $\mat{U}_{k,new}\mat{S}_{k,new}\mat{V}_{new}^T$.
}
\end{definition}

After measuring reconstruction errors, we identify the updates with \blue{high reconstruction errors} above a threshold as abnormal.
%When a newly arrived tensor is different from factor matrices of an accumulated tensor, high reconstruction errors occur.





